Rate-Interference Tradeoff in OFDM-based Cognitive Radio Networks

In cognitive radio (CR) networks, secondary users (SUs) are allowed to opportunistically access the primary users (PUs) spectrum to improve the spectrum utilization; however, this increases the interference levels at the PUs. In this paper, we consider an orthogonal frequency division multiplexing OFDM-based CR network and investigate the tradeoff between increasing the SU transmission rate (hence improving the spectrum utilization) and reducing the interference levels at the PUs. We formulate a new multiobjective optimization (MOOP) problem that jointly maximizes the SU transmission rate and minimizes its transmit power, while imposing interference thresholds to the PUs. Further, we propose an algorithm to strike a balance between the SU transmission rate and the interference levels to the PUs. The proposed algorithm considers the practical scenario of knowing partial channel state information (CSI) of the links between the SU transmitter and the PUs receivers. Simulation results illustrate the performance of the proposed algorithm and its superiority when compared to the work in the literature.

==> model_old.tex <==
% !Tex root = main_MOOP_max_rate.tex
\section{System Model} \label{sec:model}

\subsection{System Description}

Fig. \ref{fig:sys_model} depicts the system model under consideration. The available spectrum is divided into $L$ subchannels that are licensed to $L$ PUs. PUs do not necessary fully occupy their licensed spectrum temporally and/or spatially; hence, a SU may access such spectrum holes as long as no harmful interference occurs to frequency-adjacent PUs due to ACI or to other PUs operating in the same frequency band at distant location due to CCI \cite{haykin2005cognitive, Mitola1999, zhao2007survey}. Without loss of generality, we assume the SU decides to use subchannel $m$ of bandwidth $B_m$; this decision can be reached by visiting a database administrated by a government or third party, or by optionally sensing the PUs radio spectrum \cite{gao2012taxonomy, sun2012optimizing}. We assume that the SU accesses subchannel $m$ using OFDM with $N$ subcarriers.

\begin{figure}[t]
\centering
\includegraphics[width=0.50\textwidth]{sys_model}
\caption{Cognitive radio system model.}
\label{fig:sys_model}
\end{figure}

Following the common practice in the literature, we assume that the instantaneous channel gains between the SU transmitter and receiver pairs are available through a delay- and error-free feedback channel \cite{bansal2008optimal, zhang2010efficient, kang2009optimal, attar2008interference, zhao2010power,  hasan2009energy, bansal2011adaptive, kang2010optimal, ngo2010resource, kaligineedi2012power, almalfouh2011interference}. Unlike most of the work done in the literature \cite{bansal2008optimal, kang2009optimal, zhang2010efficient, attar2008interference, kang2010optimal, ngo2010resource, almalfouh2011interference}, we assume partial CSI knowledge on the links between the SU transmitter and PUs receivers (this is as estimating the instantaneous channel gains between from the SU transmitter to PUs receivers is practically challenging without the PUs cooperation). More specifically, we assume 1) knowledge of the path loss which is practically possible especially in applications with stationary nodes, where the path loss exponent and the node locations can be estimated with high accuracy \cite{salman2012low, wang2011weighted} and 2) knowledge of the path loss and the channel statistics (i.e., the fading distribution and its parameters) which is reasonable assumption for certain wireless environments, e.g., in non-line-of-sight urban environments, a Rayleigh distribution is usually assumed for the magnitude of the fading channel coefficients. The case of full CSI knowledge on the links between the SU transmitter and PUs receivers represents an upper bound on the achievable SU performance and it is provided in the numerical results section to characterize the performance loss due to the partial CSI knowledge. 

\subsection{Modeling of the CCI and ACI constraints with partial CSI knowledge}

%We assume different degree of channel information between the SU transmitter and the PU receiver. More specifically we assume the following cases: 1) knowledge of the path loss, 2) knowledge of the path loss and the mean of the distribution, 3) knowledge of the path loss and the distribution statistics, and for completeness of the presentation 4) knowledge of the path loss and the perfect CSI.

\subsubsection{Case 1---knowledge of the Path Loss} The transmit power on subchannel $m$ should be limited to a certain threshold $P_{th}^{(m)}$ to protect the $m$th distant PU receiver as follows
\begin{IEEEeqnarray}{c}
10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}} \sum_{i = 1}^{N} p_i \leq P_{th}^{(m)}, \label{eq:PL_CCI}
\end{IEEEeqnarray}
where $L(d_m)$ and FM are the distance-based path loss in dB at distance $d_m$ from the SU and the fading margin in dB, respectively and $p_i$ is the allocated power per subcarrier $i$, $i = 1, ..., N$.
To reflect the SU transmitter's power amplifier limitations and/or to satisfy regulatory maximum power limits, the total SU transmit power should be limited to a certain threshold $P_{th}$
\begin{IEEEeqnarray}{c}
\sum_{i = 1}^{N} p_i \leq P_{th}.
\end{IEEEeqnarray}
Hence, the constraint on the total transmit power is formulated as
\begin{IEEEeqnarray}{c}
\sum_{i = 1}^{N} p_i \leq \left[P_{th}, \frac{P_{th}^{(m)}}{10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}}} \right]^-.
\end{IEEEeqnarray}
To simplify the notation and without loss of generality, we assume that $\frac{P_{th}^{(m)}}{10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}}} < P_{th}$. Hence, the CCI constraint is written as
%Equation (\ref{eq:PL_CCI}) can be further written as
\begin{IEEEeqnarray}{c}
\sum_{i=1}^{N} p_i \leq P_{th}^{(m)} X_{\textup{Case 1}}^{(m)},
\end{IEEEeqnarray}
where $X_{\textup{Case 1}}^{(m)} = \frac{1}{10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}}}$ represents the channel knowledge coefficient from the SU transmitter to the $m$th PU receiver for the case of only knowing the path loss on the links between the SU transmitter to the PU receivers.

The ACI is mainly due to the frequency leakage of the SU subcarriers to the PUs receivers. This depends on the power allocated to each SU subcarrier and the spectral distance between the SU subcarriers and the PUs receivers. The ACI to the $\ell$th PU receiver should be limited to a certain threshold $P_{th}^{(\ell)}$ as \cite{weiss2004mutual}
\begin{IEEEeqnarray}{c}
10^{-0.1 \: \textup{PL}(d_{\ell})} 10^{-0.1 \: \textup{FM}} \sum_{i=1}^{N} p_i \: \varpi_i^{(\ell)} \leq P_{th}^{(\ell)}, \quad \ell = 1, ..., L, \label{eq:PL_ACI}
\end{IEEEeqnarray}
where $\varpi_i^{(\ell)} = T_{s} \: \int_{f_{i_m,\ell}-\frac{B_\ell}{2}}^{f_{i_m,\ell}+\frac{B_\ell}{2}} \textup{sinc}^2(T_{s} f) \: df$, $T_s$ is the SU OFDM symbol duration, $f_{i,\ell}$ is the spectral distance between the SU subcarrier $i$ and the $\ell$th PU  frequency band, $B_{\ell}$ is the bandwidth of $\ell$th PU, and $\textup{sinc}(x) = \frac{\sin(\pi x)}{\pi x}$. Equation (\ref{eq:PL_ACI}) can be further written as
\begin{IEEEeqnarray}{c}
\sum_{i = 1}^{N} p_i \: \varpi_i^{(\ell)} \leq P_{th}^{(\ell)} X_{\textup{Case 1}}^{(\ell)}, \quad \ell = 1, ..., L,
\end{IEEEeqnarray}
where $X_{\textup{Case 1}}^{(\ell)} = \frac{1}{10^{-0.1 \: \textup{PL}(d_{\ell})} 10^{-0.1 \: \textup{FM}}}$ is the channel knowledge coefficient from the SU transmitter to the $\ell$th PU receiver for the case of only knowing the path loss on the links between the SU transmitter and PUs receivers.


%\subsubsection{Case 2---knowledge of the path loss and the mean of the distribution}
%A non-line-of-sight propagation environment is assumed; therefore, the channel gain $\mathcal{H}_{sp}^{(m)}$ can be modeled as a zero-mean complex Gaussian random variables, and, hence, $| \mathcal{H}_{sp}^{(m)} |^2$ follows an exponential distribution \cite{proakisdigital}. In this case, the constraints are met on average as follows.
%\begin{IEEEeqnarray}{c}
%\mathbb{E} \left\{ | \mathcal{H}_{sp}^{(m)} |^2 10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}} \sum_{i = 1}^{N} p_i \right\} \leq P_{th}^{(m)}, \label{eq:mean}
%\end{IEEEeqnarray}
%after some mathematical manipulations, (\ref{eq:mean}) can be reduced to
%\begin{IEEEeqnarray}{c}
%\sum_{i = 1}^{N} p_i \leq P_{th}^{(m)} X_{\textup{Case 2}}^{(m)},
%\end{IEEEeqnarray}
%where $ X_{\textup{Case 2}}^{(m)} = \frac{(\nu^{(m)})^2}{10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}}}$ where $\frac{1}{\nu^{(m)}}$ is the mean of the exponential distribution. Similarly the ACI constraint is expressed as
%\begin{IEEEeqnarray}{c}
%\sum_{i = 1}^{N} p_i \: \varpi_i^{(\ell)} \leq P_{th}^{(\ell)} X_{\textup{Case 2}}^{(\ell)}, \quad \ell = 1, ..., L.
%\end{IEEEeqnarray}
%where $ X_{\textup{Case 2}}^{(\ell)} = \frac{(\nu^{(\ell)})^2}{10^{-0.1 \: \textup{PL}(d_{\ell})} 10^{-0.1 \: \textup{FM}}}$.


\subsubsection{Case 2---knowledge of the path loss and channel statistics}
The CCI constraint is written as
\begin{IEEEeqnarray}{c}
|\mathcal{H}_{sp}^{(m)} |^2 10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}} \sum_{i = 1}^{N} p_i \leq P_{th}^{(m)},
\end{IEEEeqnarray}
where $\mathcal{H}_{sp}^{(m)}$ is the channel gain to the distant $m$th PU receiver. Since $\mathcal{H}_{sp}^{(m)}$ is not perfectly known at the SU transmitter, the CCI constraint is limited below the threshold $P_{th}^{(m)}$ with at least a probability of $\Psi_{th}^{(m)}$. This is formulated as
\begin{IEEEeqnarray}{c}
\textup{Pr}\left( | \mathcal{H}_{sp}^{(m)} |^2 10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}} \sum_{i = 1}^{N} p_i \leq P_{th}^{(m)} \right) \geq \Psi_{th}^{(m)}. \label{eq:statistical_CCI}
\end{IEEEeqnarray}
A non-line-of-sight propagation environment is assumed; therefore, the channel gain $\mathcal{H}_{sp}^{(m)}$ can be modeled as zero-mean complex Gaussian random variables, and, hence, $| \mathcal{H}_{sp}^{(m)} |^2$ follow an exponential distribution \cite{proakisdigital}. Accordingly, the statistical constraints in (\ref{eq:statistical_CCI}) can be evaluated as
\begin{IEEEeqnarray}{c}
1 - \exp\left(- \frac{\nu^{(m)}}{10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}} \sum_{i = 1}^{N} p_i} P_{th}^{(m)}\right) \geq \Psi_{th}^{(m)}, \label{eq:statistical_CCI_1}
\end{IEEEeqnarray}
where $\frac{1}{\nu^{(m)}}$ is the mean of the exponential distribution.
%and $\sqrt{\frac{\nu^{(m)}}{2}}$ is the Rayleigh distribution parameter.
Eqn. (\ref{eq:statistical_CCI_1}) can be further written as
\begin{IEEEeqnarray}{c}
\sum_{i = 1}^{N} p_i \leq \frac{\nu^{(m)}}{\left(-\ln(1 - \Psi_{th}^{(m)})\right) 10^{- 0.1 \: \textup{PL}(d_{m})} 10^{- 0.1 \: \textup{FM}}} P_{th}^{(m)}, \label{eq:statistical_CCI_2}
\end{IEEEeqnarray}
which can be further simplified as
\begin{IEEEeqnarray}{c}
\sum_{i = 1}^{N} p_i \leq P_{th}^{(m)} X_{\textup{Case 2}}^{(m)},
\end{IEEEeqnarray}
where $X_{\textup{Case 2}}^{(m)} = \frac{\nu^{(m)}}{\left(-\ln(1 - \Psi_{th}^{(m)})\right) 10^{- 0.1 \: \textup{PL}(d_{m})} 10^{- 0.1 \: \textup{FM}}}$ is the channel knowledge coefficient from the SU transmitter to the $m$th PU receiver for the case of knowing the path loss and the channel statistics on the links between the SU transmitter and PUs receivers. Similarly the ACI constraint can be written as
\begin{IEEEeqnarray}{c}
\sum_{i = 1}^{N} p_i \: \varpi_i^{(\ell)} \leq P_{th}^{(\ell)} X_{\textup{Case 2}}^{(\ell)}, \quad \ell = 1, ..., L,
\end{IEEEeqnarray}
where $X_{\textup{Case 2}}^{(\ell)} = \frac{\nu^{(\ell)}}{\left(-\ln(1 - \Psi_{th}^{(\ell)})\right) 10^{- 0.1 \: \textup{PL}(d_{\ell})} 10^{- 0.1 \: \textup{FM}}}$ is the channel knowledge coefficient to the $\ell$th PU for the case of knowing the path loss and the channel statistics on the links between the SU transmitter and PUs receivers.


%\subsubsection{Case 3---knowledge of the path loss and the perfect CSI}
%This case is presented for completeness of the presentation and to characterize the performance loss due to the partial channel knowledge. Hence, it represents an upper bound on the SU achieved performance. Similar to the previous cases, the CCI constraint is written as
%\begin{IEEEeqnarray}{c}
%\sum_{i = 1}^{N} p_i \leq P_{th}^{(m)} X_{\textup{Case 3}}^{(m)},
%\end{IEEEeqnarray}
%where $X_{\textup{Case 3}}^{(m)} = \frac{1}{| \mathcal{H}_{sp}^{(m)} |^2 10^{-0.1 \: \textup{PL}(d_{m})} 10^{-0.1 \: \textup{FM}}}$  is the channel knowledge coefficient from the SU transmitter to the $m$th PU for case 3.  The ACI constraint is expressed as
%\begin{IEEEeqnarray}{c}
%\sum_{i = 1}^{N} p_i \: \varpi_i^{(\ell)} \leq P_{th}^{(\ell)} X_{\textup{Case 3}}^{(\ell)}, \quad \ell = 1, ..., L.
%\end{IEEEeqnarray}
%where $X_{\textup{Case 3}}^{(\ell)} = \frac{1}{| \mathcal{H}_{sp}^{(\ell)} |^2 10^{-0.1 \: \textup{PL}(d_{\ell})} 10^{-0.1 \: \textup{FM}}}$ is the channel knowledge coefficient for the $\ell$th PU for case 3. 

==> proposed.tex <==
\section{Proposed Algorithms and Complexity Analysis} \label{sec:proposed}

\subsection{Proposed Algorithms}

The proposed algorithm can be formally stated as follows:

\floatname{algorithm}{}
\begin{algorithm}
\renewcommand{\thealgorithm}{}
\caption{\textbf{$\mathbb{PA}1$: Proposed Algorithm to solve $\mathbb{OP}1$}}
\begin{algorithmic}[1]
%\small
\State \textbf{INPUT} $\sigma^2_n$, $\mathcal{H}_{i}$, $\alpha$, $\mathcal{P}_{th}^{(m)}$, $\mathcal{P}_{th}^{(\ell)}$, $X^{(m)}$, and $X^{(\ell)}$, $\ell = 1, ..., L$.
\For{$i$ = 1, ..., $N$}
\State $p_i^*$ is given by (\ref{eq:sol_op1_1}).
\EndFor
%        \algstore{myalg}
%  \end{algorithmic}
%\end{algorithm}
%
%\floatname{algorithm}{}
%\begin{algorithm}
% % \ContinuedFloat
% \renewcommand{\thealgorithm}{}
%  \caption{\textbf{$\mathbb{PA}1$: Proposed Algorithm to solve $\mathbb{OP}1$} (continued)}
%  \begin{algorithmic}
%      \algrestore{myalg}
%      \small
\If {$\sum_{i = 1}^{N} p_i^* \geq P_{th}^{(m)} X^{(m)}$ and $\sum_{i = 1}^{N} p_i^* \varpi_i^{(\ell)} < P_{th}^{(\ell)} X^{(\ell)}$}
\State $p_i^*$ is given by (\ref{eq:sol_op1_2}).
%\State $\lambda_{N+1}$ is given by (\ref{eq:lambda}).
\State $\lambda_{N+1}$ is calculated to satisfy $\sum_{i = 1}^{N} p_i^* = P_{th}^{(m)} X^{(m)}$.
\ElsIf {$\sum_{i = 1}^{N} p_i^* < P_{th}^{(m)} X^{(m)}$ and $\sum_{i = 1}^{N} p_i^* \varpi_i^{(\ell)} \geq P_{th}^{(\ell)} X^{(\ell)}$}
\State  $p_i^*$ is given by (\ref{eq:sol_op1_3}).
\State $\lambda_{N+2}^{(\ell)}$ is calculated to satisfy $\sum_{i = 1}^{N} p_i^* \varpi_i^{(\ell)} = P_{th}^{(\ell)} X^{(\ell)}$, $\ell = 1, ..., L$.
\Else \:  \textbf{if} {$\sum_{i = 1}^{N} p_i^* \geq P_{th}^{(m)} X^{(m)}$ and $\sum_{i = 1}^{N} p_i^* \varpi_i^{(\ell)} \geq P_{th}^{(\ell)} X^{(\ell)}$} \textbf{then}
\State  $p_i^*$ is given by (\ref{eq:sol_op1_4}).
\State $\lambda_{N+1}$ and $\lambda_{N+2}^{(\ell)}$ are calculated to satisfy $\sum_{i = 1}^{N} p_i^* = P_{th}^{(m)} X^{(m)}$ and $\sum_{i = 1}^{N} p_i^* \varpi_i^{(\ell)} = P_{th}^{(\ell)} X^{(\ell)}$, $\ell = 1, ..., L$, respectively.
\EndIf
\State \textbf{OUTPUT} $p_i^*$, $i$ = 1, ..., $N$.
\end{algorithmic}
\end{algorithm}

\subsection{Complexity Analysis}
%\vspace{-10pt}
The authors in \cite{palomar2005practical} showed that the Lagrange multipliers $\lambda_{N+1}$ and $\lambda_{N+2}^{(\ell)}$, $\ell = 1, ..., L$, that satisfy the CCI and ACI constraints, respectively, can be obtained with linear complexity of the number of subcarrier $N$, i.e., $\mathcal{O}(N)$. Therefore, the worst case computational complexity of the proposed algorithms to solve $\mathbb{OP}1$ and $\mathbb{OP}2$ can be analyzed as follows. Steps 2 to 4 require a complexity of  $\mathcal{O}(N)$; steps 5 to 7, 8 to 10, and 11 to 13 require a complexity of $\mathcal{O}(N^2)$. Thus, the worst case computational complexity  of the proposed algorithms to solve $\mathbb{OP}1$ and $\mathbb{OP}2$ is calculated as $\mathcal{O}(N) + \mathcal{O}(N^2) + \mathcal{O}(N^2) + \mathcal{O}(N^2) = \mathcal{O}(N^2)$.

%\newpage 
